SpikeDerain: Unveiling Clear Videos from Rainy Sequences Using Color Spike Streams

Restoring clear frames from rainy videos presents a significant challenge due to the rapid motion of rain streaks. Traditional frame-based visual sensors, which capture scene content synchronously, struggle to capture the fast-moving details of rain accurately. In recent years, neuromorphic sensors have introduced a new paradigm for dynamic scene perception, offering microsecond temporal resolution and high dynamic range. However, existing multimodal methods that fuse event streams with RGB images face difficulties in handling the complex spatiotemporal interference of raindrops in real scenes, primarily due to hardware synchronization errors and computational redundancy. In this paper, we propose a Color Spike Stream Deraining Network (SpikeDerain), capable of reconstructing spike streams of dynamic scenes and accurately removing rain streaks. To address the challenges of data scarcity in real continuous rainfall scenes, we design a physically interpretable rain streak synthesis model that generates parameterized continuous rain patterns based on arbitrary background images. Experimental results demonstrate that the network, trained with this synthetic data, remains highly robust even under extreme rainfall conditions. These findings highlight the effectiveness and robustness of our method across varying rainfall levels and datasets, setting new standards for video deraining tasks. The code will be released soon.

==> sec/0_abstract.tex <==
\begin{abstract}
Restoring clear frames from rainy videos is a significant challenge due to the rapid motion of rain streaks. Traditional frame-based visual sensors, which capture dense scene content synchronously, struggle to accurately capture the fast-moving rain details. In recent years, neuromorphic sensors have provided a new paradigm for dynamic scene perception due to their microsecond temporal resolution and high dynamic range characteristics. However, the existing multimodal methods that fuse event streams with RGB images make it difficult to cope with the complex spatiotemporal interference of raindrops in real scenes due to hardware synchronization errors and computational redundancy. In this paper, we propose a two-stage decoupled network driven by color spike streams, which can achieve spike stream reconstruction of dynamic scenes and accurate removal of rain streaks. In order to further solve the problems of data scarcity and distribution bias in real continuous rainfall scenes, we design a physically interpretable rain streak synthesis model that can generate parameterized continuous rain patterns based on arbitrary background images. Experiments show that the network trained with this synthetic data remains highly robust under extreme rainfall conditions. These results emphasize the effectiveness and robustness of our method across different rainfall levels and datasets, setting new standards for video deraining tasks.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Rainfall, as the most common severe weather phenomenon, can cause severe degradation of captured videos and images. This degradation not only reduces visual quality but also significantly affects the reliability of computer vision tasks that rely on clear input ,e.g., object detection\cite{40}, person re-identification\cite{41}. Traditional RGB cameras are limited by a fixed exposure mechanism\cite{42} and find it difficult to capture the transient motion trajectory of high-speed raindrops, resulting in a fundamental bottleneck in the recovery of details in existing frame-based video deraining methods. In recent years, neuromorphic sensors (e.g., event cameras)\cite{43,44,45} have provided a new paradigm for dynamic scene perception due to their microsecond temporal resolution and high dynamic range characteristics. However, there are still two major challenges in reconstructing rain-free images from the high-frequency asynchronous data stream of neuromorphic sensors: The event stream only records sparse events of brightness changes\cite{26}, loses absolute brightness and color information, and is difficult to distinguish between rain streaks and background textures; The existing multimodal methods\cite{46} that fuse event streams with RGB images are difficult to cope with the complex spatiotemporal interference of raindrops in real scenes due to hardware synchronization errors\cite{47} and computational redundancy.
%-------------------------------------------------------------------------

\begin{figure}[t]
\begin{center}
   \includegraphics[width=1\linewidth]{ICCV2025-Author-Kit/figure/motivation.png}
\end{center}
   \caption{Comparison between traditional video frames and spike streams. Traditional cameras, due to exposure time and fixed sampling frequency, result in dynamic blur and inter frame intervals in captured images, thereby reducing the image quality of subsequent tasks. Spike stream, with its ultra-high time resolution, can better capture high-speed information.}
\label{fig:motivation}
\end{figure}

%-------------------------------------------------------------------------
To address the above issues, this paper proposes the first single-modal rain removal framework based on a color spike stream. Unlike event cameras, spike cameras generate spike streams by continuously capturing the absolute brightness of each pixel\cite{14,17,20,24} and spike cameras with CFA\cite{23,48,49,50} can retain certain color information while acquiring spike streams. Their natural fusion of spatiotemporal continuity and multispectral information provides dual advantages for rain removal tasks: Physical consistency: The color spike stream output by a single sensor avoids cross-modal alignment errors, which is especially suitable for scenes with high-speed relative motion between rain streaks and background; Information integrity: The spike sequence simultaneously encodes the dynamic details and color distribution of the scene, effectively solving the rain streak-background confusion problem caused by color loss in traditional event stream methods.


In this paper, we design a color spike stream derain network (CSDerainNet), which maps the raw spike stream into a continuous spatiotemporal representation through spike density and color correlation, and jointly optimizes the image reconstruction and rain streak separation processes. To further solve the problems of data scarcity and distribution bias in real continuous rainfall scenes, we propose a physically interpretable rain streak synthesis model that can generate parameterized continuous rain streaks based on arbitrary background images. The model accurately simulates the spatiotemporal interaction effect between the rain streaks and the background by defining the physical properties of the raindrops, including movement direction, width, and density, significantly improving the diversity and authenticity of the synthetic data. Experiments show that the network trained with this synthetic data remains highly robust under extreme rainfall conditions. The contributions can be summarized as follows:

\begin{itemize}[left=0pt]
\item We use the spatiotemporal-spectral joint characterization capability of color spike streams to achieve single-mode spike-driven rain removal for the first time;
\item We propose a two-stage decoupled network driven by color spike streams, which can achieve spike stream reconstruction of dynamic scenes and accurate removal of rain streaks.
\item We designed a parameterized rain streak generator that can quantitatively control the physical properties of rain streaks, including direction, width, and density;
\item We have achieved significant improvements in PSNR, SSIM, and other indicators compared to SOTA methods, extensive experiments have proved the effectiveness of each module.
\end{itemize}


==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:formatting}

In this section, we briefly review some existing video-deraining methods and spike-based work as well as the development of spiking neural networks.
%-------------------------------------------------------------------------
\subsection{Video Deraining}
The key difference between video deraining and single image deraining methods is that they can exploit the temporal continuity in video sequences. Early research was laid by Garg and Nayar\cite{1,2,3,4}, who proposed a rain streak removal method based on linear spatiotemporal modeling. Later, researchers further improved the effect of video deraining by using different prior knowledge, including Fourier domain\cite{5}, geometric structure\cite{6}, directional features\cite{7}, and patch-based techniques\cite{8}. These methods reconstruct clear images in different ways.

Significant advancements in video rain removal have been achieved through computer vision and deep learning technologies. Recently, deep learning methodologies for video deraining have been proposed. Liu et al.\cite{9} proposed a method to extract representative features from adjacent frames using recurrent neural networks, while Li et al.\cite{10} used multi-scale sparse coding to represent rain streak patterns, significantly improving the deraining performance. In addition, for training without paired data, Yang et al.\cite{11} proposed a self-learning method, while Yue et al.\cite{12} further improved the video deraining effect by using semi-supervised learning through a dynamic generator. Wang et al.\cite{13} integrated synthetic models and prior knowledge, utilizing a video rain prior model, residual learning, and multi-scale feature extraction to improve rain removal performance. In this paper, we introduce the spike stream captured by a spike camera as a novel deraining input, and retain the traditional single-modal input form, reducing the difficulty of alignment and the high computational burden caused by cross-modality.
%-------------------------------------------------------------------------
\subsection{Spike-Based Vision}
Spike cameras\cite{14,15,16,17} are inspired by the retina of primates. They differ from traditional cameras in that they can generate a synchronized spike stream for each pixel with extremely low latency. Compared with event cameras, spike cameras record the absolute light intensity, making it possible to recover better texture details. With their ultra-high temporal resolution and low energy consumption, spike cameras are widely used in a variety of scenarios including object detection\cite{21,22}, super-resolution\cite{23,24,25}, dynamic deblurring\cite{26,27}, motion estimation\cite{28}, etc. 

Among them, spiking reconstruction is the basis of most visual tasks. Zhu et al.\cite{18} first proposed a method to estimate light intensity by counting the number of spikes (TFP) in a time window and analyzing the interval between adjacent spikes (TFI). Considering that TFP usually leads to blurred images and TFI leads to noisy images, TVS\cite{19,20} was later developed to improve the quality of visual reconstruction by imitating retinal processing. Using deep learning technology, Zhao et al.\cite{29} introduced Spk2ImgNet, a grayscale spike camera reconstruction network designed to gradually handle noise and blur. Zhao et al.\cite{30} proposed the network BSF to handle the fluctuations of the spike stream and achieve state-of-the-art performance. In order to enhance the robustness of the model, a self-supervised learning method based on synthetic data pairs was proposed. Chen et al.\cite{31} studied image restoration based on a blind spot network. In recent studies, a novel color spike stream has been used to preserve the color information captured by the spike camera.

%-------------------------------------------------------------------------
\subsection{Spiking Neural Networks}

Spiking neural networks (SNNs) are inspired by biological neurons in the brain and have attracted much attention for their potential in processing sparse and temporally dynamic information, such as event-based vision tasks. Traditional artificial neural networks (ANNs) rely on continuous signals and deterministic activations such as ReLUs, but SNNs use discrete binary spikes to communicate between neurons across time, which can be efficiently implemented on neuromorphic hardware\cite{32,33}. A common strategy for implementing deep SNNs is ANN-SNN conversion, where a pre-trained ANN is converted to an SNN by replacing ReLU activations with spiking neurons. However, this conversion usually results in an increase in the simulation time steps, leading to higher computational cost and latency\cite{34,35}.

Furthermore, the performance of the converted SNNs is inherently limited by the original ANNs. In contrast, directly trained SNNs have shown promise in achieving competitive performance\cite{37} while reducing the number of time steps required for simulation by leveraging alternative gradient functions or spike-timing-dependent plasticity (STDP)\cite{36}. Notably, methods such as temporal delay batch normalization (tdBN) have significantly enhanced the depth of SNN models\cite{38}, while Fang et al.\cite{39} introduced the Spike-Element-Wise (SEW) ResNet to facilitate residual learning in SNNs, a process that enables identity mapping and addresses the vanishing/exploding gradient challenge.In this paper, we incorporate SNN into the overall framework to address the challenge of video deraining. Different from the traditional event-driven method, we design a spiking deraining module to be connected in series with the original spike stream reconstruction to obtain clear rain-free images.


==> sec/3_method.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=17cm]{ICCV2025-Author-Kit/figure/framework_new.png}
\end{center}
   \caption{The architecture of the proposed Color Spike Stream Deraining Network (CSDerainNet)}
\label{fig:framework}
\end{figure*}

\section{Proposed Method}
In this section, we first introduce the working mechanism of the spike camera and the mathematical model of the video deraining task, and then we introduce the reconstruction of the color spike stream and the video deraining module in two stages. The overall framework of our method is shown in Fig.\ref{fig:framework}.

\subsection{Preliminaries}
\noindent
\textbf{Spike Camera Mechanism.}
The Spike Camera\cite{17} is a new type of neuromorphic visual sensor, and its imaging mechanism is fundamentally different from that of traditional RGB cameras and event cameras. As shown in Fig.\ref{fig:3}, each photon detector of the spike camera independently and continuously monitors the brightness of the scene. When the accumulated number of photons reaches a preset threshold, the component immediately triggers a spike signal and resets the integration circuit. This process generates an asynchronous spike stream $S(x,y,t)\in\{0,1\}^{H\times W\times 1\times T}$, where each spike simultaneously encodes the position $(x,y)$, timestamp $t$, and the absolute brightness response of the scene $I$. The mathematical formula is:
\begin{equation}S(x,y,t)=
\begin{cases}
1 & \int_{t_0}^tI(x,y,\tau)d\tau\geq\theta \\
0 & \mathrm{otherwise} 
\end{cases}
\end{equation}
where $I(x,y,\tau)$ is the instantaneous incident light intensity, and $\theta$ is the spike trigger threshold.



Compared with the global exposure mechanism of a fixed frame rate of a traditional camera \cite{42}, the microsecond time resolution of the spike camera can accurately capture the transient motion trajectory of high-speed rain streaks. At the same time, its high dynamic range adapts to the extreme lighting conditions of strong light sources and weak backgrounds at night, solving the rain streak background confusion problem caused by saturation or underexposure of traditional cameras.
%----------------------------------------------------------------------------
\begin{figure}[b]
\begin{center}
\includegraphics[width=8cm]{ICCV2025-Author-Kit/figure/spike_camera.png}
\end{center}
   \caption{Spike Camera Mechanism}
\label{fig:3}
\end{figure}

%----------------------------------------------------------------------------
\noindent
\textbf{Problem Formulation.} In traditional video deraining tasks, the input is mostly continuous video frames $I=\{I_t\}_{t=1}^n$, which are mainly composed of two parts: rain streak layer $R_t$ and clean background layer $B_t$. According to the physical model of rainfall, each frame can be considered as a superposition of clean image and rain effect, \textit{i.e.}:

\begin{equation}
I_t=B_t+R_t
\end{equation}
The video frames are captured by the spike camera to obtain a spatiotemporal continuous spike stream $S\in\{0,1\}^{H\times W\times 1\times T}$ where \textit{H} and \textit{W} signify the height and width of the image, and  \textit{T} represents the length of the spike sequence. Spike stream generation can be modeled as the following process:
\begin{equation}
S=\mathcal{G}\left(B+R\right)+N\label{con:spike_raw}
\end{equation}
\noindent
where $\mathcal{G}\left(\cdot\right)$ is the quantization function of the spike camera, which maps continuous brightness into a binary spike sequence; \textit{N} is the quantization noise introduced in the spike generation process, which can be modeled with the Poisson-Gaussian noise, \textit{i.e.}:
\begin{equation}
N\sim\mathcal{N}(0,\sigma_g^2+\sigma_p^2\cdot I_t)
\end{equation}
In order to remove rain streak noise and inevitable quantization noise from the raw spike stream as much as possible, in this paper, we propose a two-stage optimization objective for joint spike reconstruction and rain streak removal:\\
stage I: Reconstruction
\begin{equation}
    \min_{\Theta} \mathcal{L}_{\text{recon}} (F_{\Theta}(S), I)
\end{equation}\\
stage II: Deraining
\begin{equation}
     \min_{\Phi} \mathcal{L}_{\text{derain}} (G_{\Phi}(F_{\Theta}(S)), B)
\end{equation}
where $ F_{\Theta}(\cdot) $ represents the color spike stream reconstruction module, mapping $S$ to initial estimation; $G_{\Phi}$ represents deraining module, separating the background layer from the rain layer. $\mathcal{L}_{\text{recon}}$ and $\mathcal{L}_{\text{derain}}$ respectively represent reconstruction loss and rain removal loss.


\subsection{Color Spike Reconstruction}
\noindent
\textbf{Color Spike Stream with Bayer CFA.} To capture color information of dynamic scenes, the Bayer pattern color filter array (CFA) is recently employed on the spike sensor so that the spike camera can produce spike signals of different color channels at different pixels according to the Bayer pattern color arrangement.
The spike camera employs a Bayer-pattern CFA, where each pixel captures only one color channel. The mask of the filter array can be written as:
\begin{equation}
    M=M_r+M_g+M_b
\end{equation}
with $M_r,M_g, M_b\in \{0,1\}^{H\times W}$ being binary masks for the respective color channels, where 
$H$ and $W$ are the height and width of the image. In high-speed scenes with short exposures, the light intensity frames $\{\hat{I}_1,\hat{I}_2,...,\hat{I}_n\}$ captured by spike cameras are generated from dynamic scenes using a temporal window. The $t$-th latent light intensity frame $\hat{I}_t$ is related to the target scene intensity $I$ as follows:
\begin{equation}
    \hat{I}_t = M \cdot \Omega_{k \to t} \cdot I, \quad t \in \{1, 2, \dots, n\}
\end{equation}
where $I$ is the target light intensity, which is to be reconstructed from the spike frames over the temporal period, $\Omega_{k \to t}$ denotes the motion transformation matrix from the reference frame $k$ to the $t$-th frame. As shown in Fig. \ref{fig:cfa}, after obtaining potential light intensity frames containing noise, they will be processed through a spike camera imaging mechanism to generate a color spike stream. Thus, Eq.\ref{con:spike_raw} can be modified to:
\begin{equation}
S=\mathcal{G}\left(M \cdot \Omega_{k \to t} \cdot I\right)+N
\end{equation}
The spike signals generated by each channel are recorded at different positions in $S_{color}$.

\begin{figure}[t]
\begin{center}
\includegraphics[width=8cm]{ICCV2025-Author-Kit/figure/spike_cfa.png}
\end{center}
   \caption{Color Spike Stream with Bayer CFA}
\label{fig:cfa}
\end{figure}





\noindent
\textbf{Reconstruction Module.}
The reconstruction module aims to generate a clean, full-resolution color image from the Bayer-pattern spike data captured by the spike camera. This process involves handling the noise present in the spike data and predicting the missing pixels in each of the color channels. The module is designed to address both the temporal and spatial challenges posed by the Bayer pattern and the binary nature of the spike stream, which consists of \textbf{Color Spike Representation(CSR)}, \textbf{Spike Noise Estimator(SNE)} and \textbf{Color Correlation Prior(CCP)}.

Initially, the Bayer-pattern spike frames are passed through the Color Spike Representation (CSR) module. CSR is responsible for aligning the temporal features of each color channel, accounting for the motion offset between frames. By multiplying the spike frames with the Bayer mask for each color channel, we obtain the frames with missing pixels. A multi-scale 3D convolution encoder is employed to process these frames, extracting temporal features at different scales. The features are then fused using an offset-sharing deformable convolution (OSDCN) module, which learns a shared offset for each color channel, aligning the features and correcting for motion-induced misalignment across frames. The final output of CSR is a set of aligned feature blocks for each color channel, mathematically formulated as follows:
\begin{equation}
    Output = \text{Concat}\left( \text{OSDCN}\left( \text{3DEncoder}(M_c \cdot S) \right)\right)
\end{equation}
where $M_c \cdot S$ represents separating from the spike stream by color channel, $\text{3DEncoder}(\cdot )$ represents multi-scale 3D convolution encoder. 

A spike noise estimator (SNE) has been utilized in our work to estimate the noise in the spike data. Spike data is subject to various types of noise, including Poisson-Gaussian noise and quantization noise, which can severely degrade the quality of the reconstructed image. Therefore, accurate noise estimation is crucial for obtaining a high-quality reconstruction. To estimate the noise, the SNE module processes the spike frames through a residual block-based encoder. The encoder is designed to capture the noise features of the spike data for each color channel. After extracting the noise features, these are passed through a decoder to obtain global noise information. The decoder is designed to generate a comprehensive noise map that captures the noise characteristics across all color channels.

To improve the reconstruction quality further, the Color Correlation Prior (CCP) module is employed. This module leverages the inherent correlation between the color channels to refine the reconstruction, taking advantage of the fact that the three color channels share certain spatial and temporal characteristics. The CCP module begins by concatenating the noise features $N_{global}$ from the SNE module with the feature blocks $F_r,F_g,F_b $ obtained from the CSR module. This concatenation allows the CCP module to process both the color information and the noise features simultaneously, providing a richer context for the reconstruction process. The concatenated input is processed by an encoder to extract deep features, which are then decoded to refine the color details using channel correlations. The CCP module enhances the reconstruction by leveraging the correlations between color channels, improving texture and detail in the reconstruction.



 
\subsection{Video Deraining}
In this work, we propose a novel approach for video deraining by leveraging the Spiking Neural Network (SNN) framework. This method is adapted from the efficient spiking deraining network and extends it to handle continuous video inputs, where temporal dependencies between frames are crucial to accurately remove rain streaks. The method focuses on processing temporal sequences of frames to exploit the correlation between consecutive frames, improving rain streak removal without losing important video details.

\textbf{Spiking Residual Blocks.} Given a video input consisting of consecutive frames $I=\{ I_1,I_2,...,I_n\}$, where $n$ is the total number of frames, we encode each frame  $I_t$ into spike sequences using a biologically inspired encoding strategy. This converts each pixel’s intensity into a temporal spike stream, representing the changes in intensity over time. The Spiking Residual Blocks (SRB) are the core components of our deraining method. Each SRB processes the temporal spike sequences to capture and remove the rain streaks across frames. The SRB consists of \textbf{Spike Convolution Unit (SCU)}, \textbf{Mixed Attention Unit (MAU)} and \textbf{Residual Learning}.

SCU converts the spiking representation into a temporal feature map by simulating membrane potential dynamics. It captures temporal variations and rain patterns by analyzing spike responses over consecutive frames. LIF neurons have been utilized in SCU to convert input signals into spike sequences, as they better balance biological characteristics and computational complexity. The explicit dynamic equation for LIF neurons can be expressed mathematically as:
\begin{equation}
    \left\{
\begin{aligned}
    H^{t,n} &= U^{t-1,n} + \frac{1}{\tau} \left( X^{t,n} - \left( U^{t-1,n} - V_{\text{reset}} \right) \right) \\
    S^{t,n} &= \Theta\left( H^{t,n} - V_{\text{thr}} \right) \\
    U^{t,n} &= \left( \beta H^{t,n} \right) \odot \left( 1 - S^{t,n} \right) + V_{\text{reset}} S^{t,n},
\end{aligned}
\right.
\end{equation}
where $H^{t,n}$  is the membrane potential of the neuron at time $t$ and state $n$, $S^{t,n}$ represents the firing state (1 if the neuron is firing a spike; 0 otherwise), $U^{t,n}$ is the membrane potential update of neurons. In general, the neuronal membrane potential $H^{t,n}$ is determined by the membrane potential of the previous time step $U^{t-1,n}$, the input current $X^{t,n}$, and the time constant $\tau$. If the membrane potential exceeds the threshold V, the neuron will emit a spike, the spike state $S^{t,n}$ is set to 1, and the membrane potential will be reset to $V_{\text{reset}}$. Otherwise, the membrane potential will continue to update and gradually decay.

MAU is designed to improve the efficiency of spike processing by focusing on the most relevant parts of the input spike train. In traditional spike-based models, irrelevant or noisy spike events can distort the learned features, reducing the model’s ability to focus on important temporal or spatial components of the signal. The MAU addresses this by selectively applying attention mechanisms to the input spike data. The MAU combines both spatial and temporal attention mechanisms to adjust the focus of the model dynamically. The spatial attention operates on the spatial dimensions of the input (e.g., spatial locations within an image), while the temporal attention selectively focuses on relevant time steps based on the temporal dynamics of the spike events.

Residual learning helps prevent issues such as information loss or gradient vanishing, which can occur in deep networks. By introducing skip connections, it ensures that low-level features are preserved and efficiently propagated across layers. Overall, Assuming that the output of the $n$-th SRB at the $t$-th time step is $I_t$,n, the calculated process of SRB can be depicted as:
\begin{equation}
    \left\{
\begin{aligned}
    \hat{I}^{t,n}_1 &= \text{SCU} \left( \text{SCU} \left( I^{t,n-1} \right) \right),\\
    \hat{I}^{t,n}_2 &= \text{tdBN} \left( \text{Conv} \left( I^{t,n-1} \right) \right),\\
    I^{t,n} &= \text{MAU} \left( \hat{I}^{t,n}_1 + \hat{I}^{t,n}_2 \right) + I^{t,n-1},
\end{aligned}
\right.
\end{equation}
tdBN refers to threshold-dependent batch normalization, which is a normalization method designed for spiking neural networks (SNN) to address the shortcomings of traditional batch normalization (BN) in handling sparse and time-dependent data in spiking neurons. Let $x_k^t$ represent $k$-th channel feature maps of $x_t$. Then  $x_k=(x_k^1,x_k^2,...,x_k^t)$ will be normalized by:
\begin{equation}
    \left\{
\begin{aligned}
    \hat{x}_k &= \frac{\alpha V_{\text{th}} (x_k - E[x_k])}{\sqrt{Var[x_k]} + \epsilon},\\
    y_k &= \lambda_k \hat{x}_k + \beta_k,
\end{aligned}
\right.
\end{equation}
where $V_{\text{th}}$ denotes the threshold, $\alpha$ is a hyper-parameter depending on network structure, is a tiny constant, $\lambda_k$ and $\beta_k$ are two trainable parameters, $ E[x_k]$, $Var[x_k]$ are the mean and variance of $x_k$ statistically estimated over the MiniBatch.

==> sec/4_experiment.tex <==
\section{Experiments}
In this section, we conducted comprehensive experiments on commonly used benchmark datasets to evaluate the effectiveness of the proposed method. The experiment involves rigorous testing and analysis aimed at providing a comprehensive evaluation of performance.


\begin{table*}[t]
\begin{center}
\setlength{\tabcolsep}{10pt}
\begin{tabular}{ccccccccc}
  \hline
    \multirow{2}{*}{Method}
    & \multicolumn{2}{c}{NTURain} & \multicolumn{2}{c}{RainSynLight25} & \multicolumn{2}{c}{RainSynHeavy25} & \multicolumn{2}{c}{Rain100C} \\
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
    &PSNR↑&SSIM↑&PSNR↑&SSIM↑&PSNR↑&SSIM↑&PSNR↑&SSIM↑\\
    \hline
    ESTIL & 31.21& 0.927& 29.11& 0.901& 25.16& 0.795& &\\
    D3RNet& 32.53& 0.947& 28.21& 0.879& 24.65& 0.772& 34.22&0.959\\
    JORDER& 33.12& 0.955& 29.07& 0.890& 23.28& 0.751& 34.74&0.967\\
    JDNet & 32.95& 0.953& 28.87& 0.886& 24.62& 0.758& &\\
    MPEVNet& 33.49& 0.958& 30.08& 0.904& 26.01& 0.792& &\\
    J4RNet& 32.77& 0.954& 28.19& 0.880& 24.51& 0.749& 34.41&0.966\\
    SPAC& 31.74& 0.939& 25.40& 0.826& 23.73& 0.731& 33.42&0.949\\
    DetailNet& 30.34& 0.913& 27.74& 0.870& 23.07& 0.752& 32.14 & 0.921\\
    TransWeather& 33.35& 0.955& 29.06& 0.902& 25.95& 0.797& &\\
    GridFormer& 32.96& 0.954& 28.45& 0.896& 24.66& 0.724& &\\
    EHNet& \underline{34.11}& \underline{0.962}& \underline{30.63}& \underline{0.920}& \underline{26.28}& \underline{0.811}& &\\
    Ours& \textbf{37.86}& \textbf{0.970}& \textbf{34.48}& \textbf{0.954}& \textbf{30.79}& \textbf{0.899}&\textbf{39.24} &\textbf{0.985}\\
    \hline
 \end{tabular}
 \end{center}
 \caption{Quantitative comparisons on three public datasets. Best in bold is the runner-up with an underline.} 
 \label{Quantitative}
 \end{table*}

\begin{figure*}[t]
\begin{center}
\includegraphics[width=15cm]{ICCV2025-Author-Kit/figure/Qualitative.png}
\end{center}
   \caption{Visual comparison on the NTURain dataset.}
\label{fig:qualitative}
\end{figure*}


\subsection{Dataset Preparation}
\noindent
\textbf{Rain100C dataset.}In this work, in order to more conveniently obtain image sequences with continuous rain patterns, we propose a rain pattern synthesis method based on traditional additive models. By quantitatively adjusting the physical properties of rain patterns (direction, length, width, etc.), we propose a new paradigm for continuous rain pattern synthesis. Compared to traditional synthetic continuous rain patterns, our proposed model is not limited to similar backgrounds, fixed sizes, software dependencies, etc. The generated rain patterns have strong continuity and good overall integrity, and there will be no unrealistic situations such as sudden rain pattern changes or discontinuities. Based on our proposed continuous rain pattern synthesis method, the Rain100L\cite{52} background image was used to generate the Rain100C continuous synthesis rain dataset. For each background image in the dataset, 14 rain images with continuous rain patterns were generated, and the physical characteristics of the rain patterns corresponding to different background images were different.


\noindent
\textbf{RainSynLight25 and RainSynHeavy25 datasets\cite{44}.} In these two datasets, the training set contains 190 rainy/sunny video pairs, and the testing section contains 27 pairs. It should be noted that the rainy day framework is synthesized using probability models. The rain lines in the RainSynHeavy25 dataset are denser than those in the RainSynLight25 dataset, and the corresponding spike signals for both are generated by spike simulators.

\noindent
\textbf{NTURain dataset\cite{51}.} In this dataset, videos are divided into two groups: one group is captured by a slow camera, and the other group is captured by a fast camera. This dataset has 25 pairs of rainfall sequences, with clear training versions and 8 pairs of test versions. For each rainless video, Adobe After Effects synthesizes 3 or 4 rain layers based on different settings and then adds them to the video as a rainy video. The color spike stream of this dataset is also generated by a spike simulator.


\subsection{Implementation Details}
During the training process, we used the Adam optimizer in the PyTorch framework. For the reconstruction module, we first train it separately, and the CCP modules in each iteration share the same parameters. The number of input spike frames $N$ is set to 39. We randomly crop the spike frames into $64 \times 64$ patches and set the batch size to 8. For data augmentation, we randomly flip the input frames horizontally and vertically. After the reconstruction module training is completed, freeze the module and train the overall framework, where we conduct the proposed network in the PyTorch framework with an Adam optimizer and a batch size of 12, set the learning rate to $1 \times 10^{-3}$ and apply the cosine annealing strategy to steadily decrease the final learning rate to $1 \times 10^{-7}$.
Due to the lack of corresponding spike streams in the NTURain, RainSynLight25, and RainSynHeavy25 datasets, we combined a spike simulator\cite{53} with a Bayer Pattern CFA to generate corresponding color spike streams for training our model.

\subsection{Comparisons with State-of-The-Art Methods}
In this section, we compared our network with several state-of-the-art methods: ESTIL\cite{44}, D3RNet\cite{19}, JORDER\cite{52}, JDNet\cite{54}, MPEVNet\cite{43}, J4RNet\cite{55}, SPAC\cite{51}, DetailNet\cite{56}, TransWeather\cite{57}, GridFormer\cite{58}, and EHNet\cite{59}. Among them, JORDER and JDNet are single image derain methods, MPEVNet and EHNet are event-driven methods, and TransWeather and GridFormer are comprehensive models used to handle various weather conditions. We use Peak Signal to Noise Ratio (PSNR) and Structural Similarity (SSIM) as quantitative evaluation metrics. Following the previous approaches, we compute these metrics in the Y channel of the YCbCr space.

\noindent
\textbf{Quantitative Results on Synthetic Data.}
Table \ref {Quantitative} shows the quantitative results of our model and other advanced methods on three publicly available datasets and our proposed dataset Rain100C. According to the results shown in the table, our model achieved excellent performance on all four datasets compared to the baseline method. Specifically, our model outperforms all other models in terms of PSNR and SSIM. For example, on the NTURain dataset, our model achieved PSNR of 37.86 dB and SSIM of 0.970, with a PSNR improvement of 11\% compared to suboptimal results. On RainSynLight25, our model achieved PSNR and SSIM that were 8.20 dB and 0.034 higher than the second-best performing model EHNet. On the RainSynHeavy25 dataset with a dense distribution of rain streaks, our PSNR and SSIM reached 30.79 dB and 0.899, respectively, which were 17\% and 11\% higher than the suboptimal results. For the Rain100C dataset, which has richer background and wider varieties of rain pattern physical attributes, our method has also achieved far superior results compared to other advanced methodologies. These results emphasize the effectiveness and robustness of our method across different rainfall levels and datasets, setting new standards for video derain tasks.

\noindent
\textbf{Qualitative Results on Synthetic Data.}
As shown in Fig. \ref{fig:qualitative}, we conducted a qualitative analysis of the results of several methods on the NTURain dataset. The scene shown in the image was captured by a fast camera. The green box in each image represents a thicker rain streak, while the red box represents more difficult to process interlaced rain patterns. From the comparison results, it can be seen that DetailNet and SPAC can only remove a small number of rain streaks in high-speed scenes, while a large number of rain streaks still exist, which corresponds to the poor performance in the quantitative results. Although D3RNet, J4RNet, and JORDER can remove more rain streaks than the first two competitors, there are still some rain streaks. MPEVNet and EHNet achieve significantly better performance in high-speed scenarios by introducing event streams but also face challenges in different scenarios. Among all the comparison methods, Ours can obtain the best results.

\subsection{Ablation Studies}
To clarify what contributed to the superior performance of our method, we conducted ablation studies to demonstrate the effectiveness of each component. All ablation experiments were conducted on the SynHeavy25 dataset.

\begin{table}[t]
\begin{center}
\label{ablation1}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ccccc}
  \hline
    Time steps&PSNR↑&SSIM↑&FLOPs (G)&Energy (uJ)\\
    \hline
    3 & 30.30 & 0.895 & 8.479 & $1.0565\times 10^5$\\
    4 & 30.58 & 0.896 & 8.578 & $1.0690\times 10^5$\\
    5 & 30.79 & 0.899 & 8.678 & $1.0814\times 10^5$\\
    6 & 30.47 & 0.894 & 8.777 & $1.0939\times 10^5$\\
    7 & 29.72 & 0.885 & 8.877 & $1.1064\times 10^5$\\
    \hline
 \end{tabular}
 \end{center}
 \caption{Impact of different time steps on RainSynHeavy25  dataset.} 
 \label{time_step}
 \end{table}


\begin{table}[t]
\begin{center}
\label{ablation1}
\setlength{\tabcolsep}{8pt}
\begin{tabular}{cccc}
  \hline
    Reconstruction&PSNR↑&SSIM↑&LPIPS↓\\
    \hline
    TFP & 30.34 & 0.889 & 0.112 \\
    TFI & 28.32 & 0.843 & 0.171 \\
    BSN & 24.87 & 0.714 & 0.477 \\
    Ours& 30.79 & 0.899 & 0.104 \\
    \hline
 \end{tabular}
 \end{center}
 \caption{Impact of different reconstruction methods on RainSynHeavy25  dataset.} 
 \label{reconstruct}
 \end{table}

 \begin{table}[t]
\begin{center}
\label{ablation1}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{cccccccc}
  \hline
    Model&BN&tdBN&CU&SCU&PSNR↑&SSIM↑&LPIPS↓\\
    \hline
    (a)& \checkmark &            &            & \checkmark & 30.71 & 0.896 & 0.112\\
    (b)& \checkmark &            & \checkmark &            & 30.21 & 0.889 & 0.126\\
    (c)&            & \checkmark & \checkmark &            & 29.96 & 0.876 & 0.132\\
    (d)&            & \checkmark &            & \checkmark & 30.79 & 0.899 & 0.104\\
    \hline
 \end{tabular}
 \end{center}
 \caption{Quantitative ablation study on different components of our network on RainSynHeavy25 dataset.} 
 \label{design}
 \end{table}

\noindent
\textbf{The effectiveness of different time steps.} Tab. \ref{time_step}shows the performance results of the model at different time steps. According to the experimental results, it can be found that the longer the time step, the higher the quality of image restoration. This indicates that a higher time step can enhance the model to better obtain feature representations. Similarly, this has also led to a significant increase in energy costs. Considering the symmetry of time characteristics and in order to better balance performance and efficiency, we have chosen a time step of 5 as the default time step.

\noindent
\textbf{The effectiveness of different reconstruction methods.} To demonstrate the excellent performance of our reconstruction module in processing color spike streams, we have selected several common spike reconstruction methods to compare with our reconstruction module. Table \ref {reconstruct} shows the PSNR/SSIM/LPIPS of the final rain removal results using different reconstruction methods. In order to match the color spike spike of the Bayer pattern, we reconstructed the image into three channels using CFA mask. From the comparison results, it can be seen that the traditional TFP method preserves color information to a lower extent when processing color spike streams, while the BSN method, which performs better in other fields, disrupts the color correlation of different channels. Compared to other methods, the reconstruction method we use fully preserves color information and avoids color distortion during subsequent processing.

\noindent
\textbf{The effectiveness of SNN.} Next, the impact of the Spiking Neural Network (SNN) on deraining performance is explored through several ablation experiments. The results, as presented in Tab.\ref{design}, demonstrate that the introduction of spiking neurons and corresponding tdBN can effectively improve the overall rain removal performance of the network. Compared to traditional convolution operations, spiking neurons can achieve certain improvements when paired with tdBN.


==> sec/motivation.tex <==
\section{Motivation}
%这部分主要介绍关于为什么引入脉冲相机，内容可以包括脉冲相机的优势，和传统相机以及事件相机的对比分析等。

